Optical Flow Estimation using a Spatial Pyramid Network

We learn to compute optical flow by combining a classical spatial-pyramid formulation with deep learning. This estimates large motions in a coarse-to-fine approach by warping one image of a pair at each pyramid level by the current flow estimate and computing an update to the flow. Instead of the standard minimization of an objective function at each pyramid level, we train one deep network per level to compute the flow update. Unlike the recent FlowNet approach, the networks do not need to deal with large motions; these are dealt with by the pyramid. This has several advantages. First, our Spatial Pyramid Network (SPyNet) is much simpler and 96% smaller than FlowNet in terms of model parameters. This makes it more efficient and appropriate for embedded applications. Second, since the flow at each pyramid level is small (< 1 pixel), a convolutional approach applied to pairs of warped images is appropriate. Third, unlike FlowNet, the learned convolution filters appear similar to classical spatio-temporal filters, giving insight into the method and how to improve it. Our results are more accurate than FlowNet on most standard benchmarks, suggesting a new direction of combining classical flow methods with deep learning.

==> abstract.tex <==
We learn to compute optical flow by combining a classical coarse-to-fine flow approach with deep learning.
Specifically we adopt a spatial-pyramid formulation to deal with large motions.
According to standard practice, we warp one image of a pair at each pyramid level by the current flow estimate and compute an update to the flow field.
Instead of the standard minimization of an objective function at each pyramid level, we train a deep neural network at each level to compute the flow update.
Unlike the recent FlowNet approach, the networks do not need to deal with large motions; these are dealt with by the pyramid.  
This has several advantages. First the network is much simpler and much smaller; our Spatial Pyramid Network (SPyNet) is 96\% smaller than FlowNet in terms of model parameters.
Because it is so small, the method could be made to run on a cell phone or other embedded system.
Second, since the flow is assumed to be small at each level ($< 1$ pixel), a convolutional approach applied to pairs of warped images is appropriate.
Third, unlike FlowNet, the filters that we learn appear similar to classical spatio-temporal filters, possibly giving insight into how to improve the method further.
%We train the method on the same Flying Chairs dataset as FlowNet and achieve higher accuracy on the test set of most standard benchmarks (Sintel and Middlebury).  
% Additionally our method is much better at small motions than FlowNet.
%SPyNet is also much more accurate than the Classic+NL pyramid method upon which it is based.
Our results are more accurate than FlowNet in most cases and suggest a new direction of combining classical flow methods with deep learning. 
%may yield benefits over pure black-box CNN approaches.
